Inference on model parameters with many L-moments

This paper studies parameter estimation using L-moments, an alternative to traditional moments with attractive statistical properties. The estimation of model parameters by matching sample L-moments is known to outperform maximum likelihood estimation (MLE) in small samples from popular distributions. The choice of the number of L-moments used in estimation remains ad-hoc, though: researchers typically set the number of L-moments equal to the number of parameters, which is inefficient in larger samples. In this paper, we show that, by properly choosing the number of L-moments and weighting these accordingly, one is able to construct an estimator that outperforms MLE in finite samples, and yet retains asymptotic efficiency. We do so by introducing a generalised method of L-moments estimator and deriving its properties in an asymptotic framework where the number of L-moments varies with sample size. We then propose methods to automatically select the number of L-moments in a sample. Monte Carlo evidence shows our approach can provide mean-squared-error improvements over MLE in smaller samples, whilst working as well as it in larger samples. We consider extensions of our approach to the estimation of conditional models and a class semiparametric models. We apply the latter to study expenditure patterns in a ridesharing platform in Brazil.

==> plots/gev/plots/gpd/coverage_plots.tex <==

\begin{figure}[H]
	\centering
	
	
	
	\begin{subfigure}[H]{\textwidth}
		
		
		\centering
		\includegraphics[width=0.24\textwidth]{plots/gpd/coverage/coverage_gpd_N50_tau0.5_true.pdf}   \includegraphics[width=0.24\textwidth]{plots/gpd/coverage/coverage_gpd_N50_tau0.9_true.pdf}
		\includegraphics[width=0.24\textwidth]{plots/gpd/coverage/coverage_gpd_N50_tau0.99_true.pdf}   \includegraphics[width=0.24\textwidth]{plots/gpd/coverage/coverage_gpd_N50_tau0.999_true.pdf}
		\caption{$T=50$}
	\end{subfigure}
	
	
	\begin{subfigure}[H]{\textwidth}
		
		
		\centering
		\includegraphics[width=0.24\textwidth]{plots/gpd/coverage/coverage_gpd_N100_tau0.5_true.pdf}   \includegraphics[width=0.24\textwidth]{plots/gpd/coverage/coverage_gpd_N100_tau0.9_true.pdf}
		\includegraphics[width=0.24\textwidth]{plots/gpd/coverage/coverage_gpd_N100_tau0.99_true.pdf}   \includegraphics[width=0.24\textwidth]{plots/gpd/coverage/coverage_gpd_N100_tau0.999_true.pdf}
		\caption{$T=100$}
	\end{subfigure}
	
	
	\begin{subfigure}[H]{\textwidth}
		
		
		\centering
		\includegraphics[width=0.24\textwidth]{plots/gpd/coverage/coverage_gpd_N500_tau0.5_true.pdf}   \includegraphics[width=0.24\textwidth]{plots/gpd/coverage/coverage_gpd_N500_tau0.9_true.pdf}
		\includegraphics[width=0.24\textwidth]{plots/gpd/coverage/coverage_gpd_N500_tau0.99_true.pdf}   \includegraphics[width=0.24\textwidth]{plots/gpd/coverage/coverage_gpd_N500_tau0.999_true.pdf}
		\caption{$T=500$}
	\end{subfigure}
	
	\caption{gpd: coverage of confidence intervals based on the true sampling variance.}
	\label{fig:gpd_coverage_true}
\end{figure}

\begin{figure}[H]
	\centering
	
	
	
	\begin{subfigure}[H]{\textwidth}
		
		
		\centering
		\includegraphics[width=0.24\textwidth]{plots/gpd/coverage/length_gpd_N50_tau0.5_true.pdf}   \includegraphics[width=0.24\textwidth]{plots/gpd/coverage/length_gpd_N50_tau0.9_true.pdf}
		\includegraphics[width=0.24\textwidth]{plots/gpd/coverage/length_gpd_N50_tau0.99_true.pdf}   \includegraphics[width=0.24\textwidth]{plots/gpd/coverage/length_gpd_N50_tau0.999_true.pdf}
		\caption{$T=50$}
	\end{subfigure}
	
	
	\begin{subfigure}[H]{\textwidth}
		
		
		\centering
		\includegraphics[width=0.24\textwidth]{plots/gpd/coverage/length_gpd_N100_tau0.5_true.pdf}   \includegraphics[width=0.24\textwidth]{plots/gpd/coverage/length_gpd_N100_tau0.9_true.pdf}
		\includegraphics[width=0.24\textwidth]{plots/gpd/coverage/length_gpd_N100_tau0.99_true.pdf}   \includegraphics[width=0.24\textwidth]{plots/gpd/coverage/length_gpd_N100_tau0.999_true.pdf}
		\caption{$T=100$}
	\end{subfigure}
	
	
	\begin{subfigure}[H]{\textwidth}
		
		
		\centering
		\includegraphics[width=0.24\textwidth]{plots/gpd/coverage/length_gpd_N500_tau0.5_true.pdf}   \includegraphics[width=0.24\textwidth]{plots/gpd/coverage/length_gpd_N500_tau0.9_true.pdf}
		\includegraphics[width=0.24\textwidth]{plots/gpd/coverage/length_gpd_N500_tau0.99_true.pdf}   \includegraphics[width=0.24\textwidth]{plots/gpd/coverage/length_gpd_N500_tau0.999_true.pdf}
		\caption{$T=500$}
	\end{subfigure}
	
	\caption{gpd: relative length of confidence (vis-à-vis the unfeasible MLE-based CI) intervals based on the true sampling variance.}
	\label{fig:gpd_length_true}
\end{figure}


\begin{figure}[H]
	\centering
	
	
	
	\begin{subfigure}[H]{\textwidth}
		
		
		\centering
		\includegraphics[width=0.24\textwidth]{plots/gpd/coverage/coverage_gpd_N50_tau0.5_est.pdf}   \includegraphics[width=0.24\textwidth]{plots/gpd/coverage/coverage_gpd_N50_tau0.9_est.pdf}
		\includegraphics[width=0.24\textwidth]{plots/gpd/coverage/coverage_gpd_N50_tau0.99_est.pdf}   \includegraphics[width=0.24\textwidth]{plots/gpd/coverage/coverage_gpd_N50_tau0.999_est.pdf}
		\caption{$T=50$}
	\end{subfigure}
	
	
	\begin{subfigure}[H]{\textwidth}
		
		
		\centering
		\includegraphics[width=0.24\textwidth]{plots/gpd/coverage/coverage_gpd_N100_tau0.5_est.pdf}   \includegraphics[width=0.24\textwidth]{plots/gpd/coverage/coverage_gpd_N100_tau0.9_est.pdf}
		\includegraphics[width=0.24\textwidth]{plots/gpd/coverage/coverage_gpd_N100_tau0.99_est.pdf}   \includegraphics[width=0.24\textwidth]{plots/gpd/coverage/coverage_gpd_N100_tau0.999_est.pdf}
		\caption{$T=100$}
	\end{subfigure}
	
	
	\begin{subfigure}[H]{\textwidth}
		
		
		\centering
		\includegraphics[width=0.24\textwidth]{plots/gpd/coverage/coverage_gpd_N500_tau0.5_est.pdf}   \includegraphics[width=0.24\textwidth]{plots/gpd/coverage/coverage_gpd_N500_tau0.9_est.pdf}
		\includegraphics[width=0.24\textwidth]{plots/gpd/coverage/coverage_gpd_N500_tau0.99_est.pdf}   \includegraphics[width=0.24\textwidth]{plots/gpd/coverage/coverage_gpd_N500_tau0.999_est.pdf}
		\caption{$T=500$}
	\end{subfigure}
	
	\caption{gpd: coverage of confidence intervals that rely on an estimator of the asymptotic variance.}
	\label{fig:gpd_coverage_est}
\end{figure}


\begin{figure}[H]
	\centering
	
	
	
	\begin{subfigure}[H]{\textwidth}
		
		
		\centering
		\includegraphics[width=0.24\textwidth]{plots/gpd/coverage/length_gpd_N50_tau0.5_est.pdf}   \includegraphics[width=0.24\textwidth]{plots/gpd/coverage/length_gpd_N50_tau0.9_est.pdf}
		\includegraphics[width=0.24\textwidth]{plots/gpd/coverage/length_gpd_N50_tau0.99_est.pdf}   \includegraphics[width=0.24\textwidth]{plots/gpd/coverage/length_gpd_N50_tau0.999_est.pdf}
		\caption{$T=50$}
	\end{subfigure}
	
	
	\begin{subfigure}[H]{\textwidth}
		
		
		\centering
		\includegraphics[width=0.24\textwidth]{plots/gpd/coverage/length_gpd_N100_tau0.5_est.pdf}   \includegraphics[width=0.24\textwidth]{plots/gpd/coverage/length_gpd_N100_tau0.9_est.pdf}
		\includegraphics[width=0.24\textwidth]{plots/gpd/coverage/length_gpd_N100_tau0.99_est.pdf}   \includegraphics[width=0.24\textwidth]{plots/gpd/coverage/length_gpd_N100_tau0.999_est.pdf}
		\caption{$T=100$}
	\end{subfigure}
	
	
	\begin{subfigure}[H]{\textwidth}
		
		
		\centering
		\includegraphics[width=0.24\textwidth]{plots/gpd/coverage/length_gpd_N500_tau0.5_est.pdf}   \includegraphics[width=0.24\textwidth]{plots/gpd/coverage/length_gpd_N500_tau0.9_est.pdf}
		\includegraphics[width=0.24\textwidth]{plots/gpd/coverage/length_gpd_N500_tau0.99_est.pdf}   \includegraphics[width=0.24\textwidth]{plots/gpd/coverage/length_gpd_N500_tau0.999_est.pdf}
		\caption{$T=500$}
	\end{subfigure}
	
	\caption{gpd: relative length (vis-à-vis the unfeasible MLE-based CI) of confidence intervals that rely on an estimator of the asymptotic variance.}
	\label{fig:gpd_length_est}
\end{figure}





\begin{figure}[H]
	\centering
	
	
	
	\begin{subfigure}[H]{\textwidth}
		
		
		\centering
		\includegraphics[width=0.32\textwidth]{plots/gpd/coverage/coverage_gpd_N50_tau0.9_art_corr.pdf}
		\includegraphics[width=0.32\textwidth]{plots/gpd/coverage/coverage_gpd_N50_tau0.99_art_corr.pdf}   \includegraphics[width=0.32\textwidth]{plots/gpd/coverage/coverage_gpd_N50_tau0.999_art_corr.pdf}
		\caption{$T=50$}
	\end{subfigure}
	
	
	\begin{subfigure}[H]{\textwidth}
		
		
		\centering
		\includegraphics[width=0.32\textwidth]{plots/gpd/coverage/coverage_gpd_N100_tau0.9_art_corr.pdf}
		\includegraphics[width=0.32\textwidth]{plots/gpd/coverage/coverage_gpd_N100_tau0.99_art_corr.pdf}   \includegraphics[width=0.32\textwidth]{plots/gpd/coverage/coverage_gpd_N100_tau0.999_art_corr.pdf}
		\caption{$T=100$}
	\end{subfigure}
	
	\caption{gpd: coverage of unfeasible confidence intervals that rely on rescaled estimators of the asymptotic variance.}
	\label{fig:gpd_coverage_rescale}
\end{figure}







\begin{figure}[H]
	\centering
	
	
	
	\begin{subfigure}[H]{\textwidth}
		
		
		\centering
		\includegraphics[width=0.32\textwidth]{plots/gpd/coverage/coverage_gpd_N50_tau0.9_correct.pdf}
		\includegraphics[width=0.32\textwidth]{plots/gpd/coverage/coverage_gpd_N50_tau0.99_correct.pdf}   \includegraphics[width=0.32\textwidth]{plots/gpd/coverage/coverage_gpd_N50_tau0.999_correct.pdf}
		\caption{$T=50$}
	\end{subfigure}
	
	
	\begin{subfigure}[H]{\textwidth}
		
		
		\centering
		\includegraphics[width=0.32\textwidth]{plots/gpd/coverage/coverage_gpd_N100_tau0.9_correct.pdf}
		\includegraphics[width=0.32\textwidth]{plots/gpd/coverage/coverage_gpd_N100_tau0.99_correct.pdf}   \includegraphics[width=0.32\textwidth]{plots/gpd/coverage/coverage_gpd_N100_tau0.999_correct.pdf}
		\caption{$T=100$}
	\end{subfigure}
	
	
	\caption{gpd: coverage of feasible confidence intervals that rely on corrected quantiles.}
	\label{fig:gpd_coverage_correct}
\end{figure}




\begin{figure}[H]
	\centering
	
	
	
	\begin{subfigure}[H]{\textwidth}
		
		
		\centering
		\includegraphics[width=0.32\textwidth]{plots/gpd/coverage/length_gpd_N50_tau0.9_correct.pdf}
		\includegraphics[width=0.32\textwidth]{plots/gpd/coverage/length_gpd_N50_tau0.99_correct.pdf}   \includegraphics[width=0.32\textwidth]{plots/gpd/coverage/length_gpd_N50_tau0.999_correct.pdf}
		\caption{$T=50$}
	\end{subfigure}
	
	
	\begin{subfigure}[H]{\textwidth}
		
		
		\centering
		\includegraphics[width=0.32\textwidth]{plots/gpd/coverage/length_gpd_N100_tau0.9_correct.pdf}
		\includegraphics[width=0.32\textwidth]{plots/gpd/coverage/length_gpd_N100_tau0.99_correct.pdf}   \includegraphics[width=0.32\textwidth]{plots/gpd/coverage/length_gpd_N100_tau0.999_correct.pdf}
		\caption{$T=100$}
	\end{subfigure}
	
	
	
	
	\caption{GPD: relative length (vis-à-vis the unfeasible MLE-based CI that relies on the true sampling variance) of feasible confidence intervals that rely on corrected quantiles.}
	\label{fig:gpd_length_correct}
\end{figure}


